Nonlinear electro-elastic finite element analysis with neural network constitutive models

In the present work, the applicability of physics-augmented neural network (PANN) constitutive models for complex electro-elastic finite element analysis is demonstrated. For the investigations, PANN models for electro-elastic material behavior at finite deformations are calibrated to different synthetically generated datasets, including an analytical isotropic potential, a homogenised rank-one laminate, and a homogenised metamaterial with a spherical inclusion. Subsequently, boundary value problems inspired by engineering applications of composite electro-elastic materials are considered. Scenarios with large electrically induced deformations and instabilities are particularly challenging and thus necessitate extensive investigations of the PANN constitutive models in the context of finite element analyses. First of all, an excellent prediction quality of the model is required for very general load cases occurring in the simulation. Furthermore, simulation of large deformations and instabilities poses challenges on the stability of the numerical solver, which is closely related to the constitutive model. In all cases studied, the PANN models yield excellent prediction qualities and a stable numerical behavior even in highly nonlinear scenarios. This can be traced back to the PANN models excellent performance in learning both the first and second derivatives of the ground truth electro-elastic potentials, even though it is only calibrated on the first derivatives. Overall, this work demonstrates the applicability of PANN constitutive models for the efficient and robust simulation of engineering applications of composite electro-elastic materials.

==> chapter/inv_derivs.tex <==

\section{Polyconvexity of the adapted transversely isotropic invariants}\label{app:invs}
\renewcommand{\arraystretch}{2}
\begin{table}
\centering
\begin{tabular}{| l | l |c|c|c| } 
\hline
 \cellcolor[gray]{.7} & \cellcolor[gray]{.9} $\square$ & \cellcolor[gray]{.9} $\dfrac{\partial \square}{\partial \vect{F}}$& \cellcolor[gray]{.9} $\dfrac{\partial \square}{\partial \vect{d}_0}$
 \\[1ex]
\hline
%\multirow{3}{5em}{} 
 \cellcolor[gray]{.9} & $I_1 := \norm{\vect{F}}^2=\tr \vect{C}$ & $2\vect{F}$& $\vect{0}$\\ 
 \cellcolor[gray]{.9} & $I_2 := \norm{\vect{H}}^2=\tr(\cof \vect{C})$ & $2\bF\left(I_1 \bI - \bC\right)$ &$\vect{0}$\\ 
 \cellcolor[gray]{.9} & $J := \det \vect{F}$&  $\cof \vect{F}$&$\vect{0}$\\ 
 \cellcolor[gray]{.9} &$I_4:=\norm{\vect{d}_0}^2$ & $\vect{0}$&$2\vect{d}_0$\\ 
 \cellcolor[gray]{.9} &$I_5:=\norm{\vect{d}}^2=\norm{\vect{F}\vect{d}_0}^2$  &$ 2\vect{F}(\vect{d}_0\otimes\vect{d}_0)$&$2\vect{C}\vect{d}_0$\\ 
 \cellcolor[gray]{.9} &$I_5^*:=J^{-1}\,I_5$  &$ 2\,J^{-1}\,\vect{F}(\vect{d}_0\otimes\vect{d}_0)-I_5\,J^{-2}\,\cof\bF$&$2\vect{C}\vect{d}_0$\\ 
 \multirow{-6}{6em}{\cellcolor[gray]{.9}Isotropy} & $J^*:=-J$ & &\\
\hline
 \cellcolor[gray]{.9} & $J_1 :=\norm{\vect{F}\vect{G}}^2= \tr(\vect{C}\vect{G})$ & $2\vect{F}\vect{G}$& $\vect{0}$\\ 
 \cellcolor[gray]{.9} & $J_2 :=\norm{\vect{H}\vect{G}}^2=\tr(\cof(\vect{C}) \bG)$ &  $2\vect{F}\left(J_2\vect{C}^{-1}- \cof(\vect{C}) \vect{G}\vect{C}^{-1}\right)$ & $\vect{0}$\\ 
 \cellcolor[gray]{.9} & $J_3 := \tr\left(\left(\vect{d}_0\otimes\vect{d}_0\right)\vect{G}\right)$ & $\vect{0}$&$2\vect{G}\vect{d}_0$ \\
 \cellcolor[gray]{.9} & $J_1^* :=I_1-J_1$ && \\ 
 \cellcolor[gray]{.9} & $J_2^* :=I_2-J_2$ &   & \\ 
\multirow{-6}{6em}{\cellcolor[gray]{.9}Transverse isotropy} & $J_3^*:=I_4-J_3$&&
\\[1ex]
\hline
\end{tabular}
\caption{Invariants and their partial derivatives. The derivatives of the extended invariants, denoted by $^*$, follow from the remaining invariants. The structural tensor $\vect{G}$ is defined in \cref{def:G}.}
\label{tab:invs}\end{table}

In \cref{tab:invs}, the invariants and their partial derivatives used throughout this work are provided. 
%
\begin{definition}[\textbf{Structural tensor}]\label{def:G}
With the preferred direction $\vect{n}$ and $\norm{\vect{n}}=1$, the transversely isotropic structural tensor used throughout this work is defined as 
%
\begin{equation}
    \vect{G}:=\vect{n}\otimes \vect{n}\,.
\end{equation}
%
This implies $\vect{G}\vect{G}=\vect{G},\vect{G}^T=\vect{G},\norm{\vect{G}}=1$, and p.s.d. of $\vect{G}$.
\end{definition}
%
From this we can directly achieve the different notations of, e.g., $J_1$ as
%
\begin{equation}
\begin{aligned}
    J_1=\norm{\bF{\bG}}^2&=\tr\left(\left(\bF{\bG}\right)^T\bF{\bG}\right)
=\tr\left({\bG}^T\bF^T\bF{\bG}\right)
    \\
    &=\tr\left(\bC{\bG}{\bG}\right)
=\tr\left(\bC{\bG}\right)
    \end{aligned}
\end{equation}
%
where we made use of
%
\begin{equation}
    \norm{\bA}^2=\bA:\bA=\tr\left(\bA^T\bA\right)\,.
\end{equation}
%
For a proof of polyconvexity of the invariants, see e.g.~\cite{Schroeder2003,Ebbing2010}. For the convenience of the reader, polyconvexity proofs of the adapted invariants are shortly discussed.
%
\begin{theorem}
With $\vect{G}$ as defined in \cref{def:G}, the function
%
\begin{equation}
    f:\bbR^{3\times 3}\rightarrow \bbR,\quad \bA\mapsto f(\bA)=\norm{\bA}^2-\norm{\bA\bG}^2
\end{equation}
%
is convex in the components of $\bA$.
\end{theorem}
%
\begin{proof}
The second derivative of $f$ w.r.t. $\bA$ is given as
%
\begin{equation}
    \frac{\partial f}{\partial A_{ij}\partial A_{kl}}=2\delta_{ik}\delta_{jl}-2\delta_{ik}G_{lj}\,.
\end{equation}
Applying the test matrix $\bB\in\bbR^{3\times 3}$ on this Hessian yields
%
\begin{equation}
    \begin{aligned}
%    B_{ij}B_{kl}2\left(\delta_{ik}\delta_{jl}-\delta_{ik}G_{lj}\right)&=2\left(B_{kj}B_{jk}^T- B_{kl}G_{lj}B_{jk}^T\right)
 %   \\
    %&=
    2\tr\bB\bB^T-2 \tr \bB\bG\bB^T\geq 0\,.
    \end{aligned}
\end{equation}
%
%Thus, we have to show that the inequality
%
%\begin{equation}\label{ineq}
%    \tr\vect{B}^T\vect{B}\geq  \tr\vect{B}^T\vect{B}\vect{G}
%\end{equation}
%holds. 
This inequality is fulfilled as
%
\begin{equation}
    \begin{aligned}
         \norm{\vect{B}}^2= \norm{\vect{B}}^2 \norm{\vect{G}}^2\geq\norm{\vect{B}\vect{G}}^2\,
         \\
         \Longleftrightarrow
         \\
             \tr\vect{B}\vect{B}^T\geq  \tr\vect{G}^T\vect{B}^T\vect{B}\vect{G}=\tr\vect{B}\vect{G}\vect{B}^T\,.
    \end{aligned}
\end{equation}
%
\end{proof}
%
\begin{corollary}
The invariants $J_1^*,J_2^*$ as defined in \cref{tab:invs} are polyconvex, which immediately follows by setting $\vect{A}=\vect{F},\vect{A}=\vect{H}$. 
\end{corollary}

\begin{theorem}
With $\vect{G}$ as defined in \cref{def:G}, the function
%
\begin{equation}
    f:\bbR^{3}\rightarrow \bbR,\quad \ba\mapsto f(\ba)=\tr\left(\ba\otimes\ba\right)-\tr\left(\left(\ba\otimes\ba\right)\bG\right)
\end{equation}
%
is convex in the components of $\ba$.
\end{theorem}
\begin{proof}
We have to show the p.s.d. of the Hessian \cDK{We can directly show the p.s.d. of thie adapted structural tensor $\bI- \bG$, then the proof can be applied for all adapted invariants.}
%
\begin{equation}
\begin{aligned}
     %   \frac{\partial^2 f(\ba)}{\partial a_i\partial a_j}=2\left(\delta_{ij}- G_{ij}\right)
     %   \\
     %   \Longleftrightarrow
     %   \\
        \frac{\partial^2 f(\ba)}{\partial \ba \partial \ba}=2(\bI- \bG)\,.
        \end{aligned}
\end{equation}
%
which, with the test vector $\bh\in\bbR^3$, is equal to the inequality
%
\begin{equation}
\begin{aligned}
%    h_ih_j\delta_{ij}- h_ih_jG_{ij}\geq 0
%    \\
%    \Longleftrightarrow
%    \\
    \tr\left(\bh\otimes\bh\right)- \tr \left(\left(\bh\otimes\bh\right)\bG\right)\geq 0\,.
    \end{aligned}
\end{equation}
%
With $\bH:=\bh\otimes\bh$ we may reformulate this as
%
\begin{equation}\label{eq:ineq_vec}
    \tr\vect{H}\geq  \tr\vect{H}\vect{G}\,.
\end{equation}
%
As $\bH$ is p.s.d., we may apply the Cholesky decomposition $\bH=\vect{H}'{\vect{H}}'^T$ \cite[Corollary 7.2.9]{horn2013}.
%
%Then, we may express the inequality as
%
%\begin{equation}
%    \tr\vect{H}'{\vect{H}}'^T\geq  \tr\vect{H}'{\vect{H}}'^T\bG\,.
%\end{equation}
%
Then, it holds that
%
\begin{equation}
    \begin{aligned}
 \norm{{\vect{G}}}^2    \norm{{\vect{H}}'}^2    \geq  \norm{\vect{G}{\vect{H}}'}^2 
        \\
        \Longleftrightarrow
        \\
      \tr\vect{H}\geq  \tr\left(\vect{G}{\vect{H}'}{\vect{H}'}^T\bG^T\right)=\tr\vect{H}\vect{G}\,.
    \end{aligned}
\end{equation}
\end{proof}

\begin{theorem}
Consider the tensor-valued function of a tensor
%
\begin{equation}
    \vect{A}:\bbR^{3\times 3}\rightarrow\bbR^{3\times 3},\quad \vect{B}\mapsto\vect{A}\left(\vect{B}\right)\,.
\end{equation}
%
When $\vect{G}\in\bbR^{3\times 3}$ is p.s.d, then
%
\begin{equation}
    \gamma:=\tr\left[\vect{A}\left(\vect{B}\right)\,\vect{G}\right]
\end{equation}
\end{theorem}

